Tactile-Filter: Interactive Tactile Perception for Part Mating

Humans rely on touch and tactile sensing for a lot of dexterous manipulation tasks. Our tactile sensing provides us with a lot of information regarding contact formations as well as geometric information about objects during any interaction. With this motivation, vision-based tactile sensors are being widely used for various robotic perception and control tasks. In this paper, we present a method for interactive perception using vision-based tactile sensors for a part mating task, where a robot can use tactile sensors and a feedback mechanism using a particle filter to incrementally improve its estimate of objects (pegs and holes) that fit together. To do this, we first train a deep neural network that makes use of tactile images to predict the probabilistic correspondence between arbitrarily shaped objects that fit together. The trained model is used to design a particle filter which is used twofold. First, given one partial (or non-unique) observation of the hole, it incrementally improves the estimate of the correct peg by sampling more tactile observations. Second, it selects the next action for the robot to sample the next touch (and thus image) which results in maximum uncertainty reduction to minimize the number of interactions during the perception task. We evaluate our method on several part-mating tasks with novel objects using a robot equipped with a vision-based tactile sensor. We also show the efficiency of the proposed action selection method against a naive method. See supplementary video at https://www.youtube.com/watch?v=jMVBg_e3gLw .

==> rebuttal.tex <==
\clearpage
\subsection{Rebuttal}

\textbf{MR}
\begin{enumerate}
    \item Done: There is no comparison with a similar work using TacTip on large object identification strategy (contour following) using touch-only information (10.1109/LRA.2019.2899192).
    \item Done: It is unclear how the method can be used for planning the motion of the robot under real mating tasks. In the video, such demonstrations are shown, but there is no description in the paper. Computational cost, sampling time, and speed of the mating tasks in real-time would be of high interest.
    \item Done: Data acquisition process is a bit exhaustive. How about using a simulation experiment to collect data or the Sim2Real process?
\end{enumerate}

\textbf{R1}
\begin{enumerate}
    \item Done: The method is highly specific to the described task and does not address how the final control problem can be solved; i.e., once the hole has been localized, how can the peg be inserted assuming that there is still uncertainties and noise in data.
    \item N/A: Section V.E does not seem to be showing the results using the proposed method.
    \item Done: Some results shown in the video are not presented in the paper. The authors must provide information about how the final task was performed.
\end{enumerate}

\textbf{R2}
\begin{enumerate}
    \item Done: the introduction part has a lot of repeat description (not from the words but from the meaning), and lots of information is not useful. please avoid it and remove the unnecessary text.
    \item ToDo: Related work is not presented well. It can not stimulate the highlight of the proposed approach.
    \item Done: The application peg-in-hole is more complex than the letter matching. Perhaps authors can focus on their algorithm than discussing too detailed applications.
    \item Done: This reviewer does not fully understand the procedure of how to use the proposed approach for peg-in-hole. there is a gap between principle and application.
    \item ToDo: Better to use an abstract symbol to explain the scientific question that this paper is focusing on.
    \item N/A: In Sec IV A, suggest adding the explanation "how the dataset is represented", "how belief is represented"
    \item N/A: In Sec IV B, the impression of this reviewer for the hypothesis is defined like the belief of contour map, right? It is really confusing for me with the current description.
    \item N/A: When the particle filter is used, perhaps it is good to use terminology from that domain. e.g. the particle is represented as a state, and there is a relevant value for the particle, named "weight".
    \item Done: Many places in this section and Sec IV.C authors mentioned previously collected images, not clear what is "previous".
    \item Done: Sec V A. When authors sample the data. It is not clear to this reviewer why to use a maze in which no alphabet appears.
    \item Done: Sec V B. what is the motivation to test a small object if the authors plan to propose an exploration action strategy?
    \item Done: Sec V. C, why are only 12 alphabets used but Sec V. B uses 24 alphabets?
    \item Done: Sec V. E, an practical application tactile image is good. However, this reviewer does not find a strong connection between this application and the proposed highlight in the paper.
    \item ToDo: on page 3, figure 4 appears before figure 2.
\end{enumerate}

\textbf{R3}
\begin{enumerate}
    \item Done: Related work / Novelty: In the Related Work section, the paper mostly mentioned vision-based tactile sensors, interactive perception using vision, and part insertion, which are related, but not sufficient to bring out the novelty of the current work (the most relevant study mentioned is only [35]). The contributions of the paper are mainly focused on the identification of mating parts, that can facilitate the insertion or assembly of objects to be mated. Thus, the study turns out to be developing a new method for the identification of object pairs (i.e., peg and hole), using interactive tactile perception, but not a process of mating or inserting the two parts. However, the paper compared with previous studies on part insertion with the correction of pose error, which is not quite comparable. Thus, there should be a more thorough literature review of more relevant papers on object identification based on active tactile exploration. This would clarify the novelty of this paper, which is not so transparent in the current manuscript.
    \item Done: Practicability: When it comes to assembly tasks, the accurate identification of mating parts and their precise localization should be reflected by the success of inserting the two parts. However, a quantitative evaluation of this issue has not been conducted (albeit some demonstrations of the insertion are shown in the video supplementary). As a result, it is still questionable whether the accuracy of object localization obtained using Tactile-Filter is sufficient for the insertion tasks which often encounter situations where objects to be mated are fabricated with low tolerance. Moreover, with the current setup of the tactile sensors for active tactile interaction during the identification phase (only one embedded sensor for perception), it is not practical to manipulate the identified peg and insert it into the corresponding hole in one go after the identification phase (probably an auxiliary mechanism has to be introduced).
    \item Done: Generalization: The proposed method is only verified on a simple classification of alphabetical characters, although it is shown to be possible to generalize to the identification of electrical connector-socket pairs; however, the result is not sound and questionable. Thus, the extendibility of this method to real-world objects needs to be thoroughly elaborated.
    \item Done: (Section II. Related work) Conduct a more thorough literature review on relevant works of object identification and pose estimation via tactile exploration in order to bring out and clarify the novelty of this work.
    \item Done: Section II. Related work) The author claimed that “We believe that such a method might be more useful for assembly tasks with delicate objects or in cases with very low tolerance.”. However, experiments to substantiate this statement have not been conducted. Thus, unless the authors can justify the claim via experiments, it should not be included in the paper.
    \item Done: (Algorithm 1. Tactile-Filter) There are several omissions in algorithm 1: the probability threshold ($delta_prob$) to break the current loop should also be included as an argument of the input. Also, there should be an expression to select the most probable particle inside the loop in order to define the optimal action at every time step t. Moreover, the equation to update the posterior of each category from the particles is found nowhere in the paper.
    \item Done: (Section IV. C) Despite being mentioned in the paper, it is still not so clear to me how the authors obtained the set of possible actions A from which the optimal is selected. The clarification of this would further improve the soundness of this method.
    \item Done: (Section V.C. Settings) In the first paragraph, the symbol that denotes the threshold to stop the iteration is different from the one defined in Algorithm 1, and coincident with the threshold to select the range of possible actions in Section IV. C. The authors are encouraged to check mathematical notions/symbols carefully.
    \item Done: Regarding the evaluation of multiple touch experiments with large objects, the number of contacts in cases of Pixel and MoCo baselines failed to mention. Or was it only evaluated with a single touch? If it was the latter, why would the performance of the Pixel strategy be better than that of the previous experiment with small objects? Was that result obtained by chance? The authors should give a discussion on this.
    \item Done: In the experiment with small objects, the author designed the experiment with 24 alphabet characters for the classification, however, it was reduced to only 12 characters for the experiment with large objects. What is the underlying reason behind this? Does the performance become worse the larger the number of object categories?
    \item N/A: In the evaluation of industrial connectors, the results (Table III) only show the classification accuracy of baseline methods (i.e., Pixel, Moco). How is the performance of the authors’ method (Tactile-Filter)? It would be better if the authors designed the experiment in this case similar to previous ones, and also reported the results with localization accuracy. This would help justify the generalizable of this method.
    \item Done: It turns out that the method can only infer the object poses within the range of integer values since the set of peg images is collected only with the discrete integer values of locations and orientations of the robotic hand. The proposed Tactile-Filter seems not to be able to interpolate these values during the tactile exploration procedure. However, why can the results yield the submillimeter accuracy in object localization (Table 1 and Table 2)? Otherwise, please point out specifically where in the procedure the interpolated locations and orientations (with real numbers) can be obtained.
    \item Done: Last but not least, regarding the processing time, how long does it to from the current touch to the next one and for the whole identification process? This would form the baseline for the comparison to other works.
\end{enumerate}

\clearpage
\subsection{Author feedback -- Clarification Requests --}

We would like to thank the reviewers for their insightful comments, and respectfully reinforce that our paper presents a novel method using contrastive learning, particle filtering, and tactile sensing to allow probabilistic perception. We have provided experiments with a physical setup to validate the proposed novelty. Also, we would like to add that all the test objects (i.e., all the alphabet characters \& connectors) are novel and were not used for training for the contrastive learning model. We address some concerns below, and we will revise our manuscript to include all comments.

[TacTip comparison]
We want to clarify that the objective of the TacTip work is edge perception and contour following, while our primary objective is to identify and localize novel parts that fit together. We compared our method to a closer work, Tac2Pose ([3] in manuscript), denoted as "MoCo" in the paper and demonstrated our method exhibits superior performance. Tac2Pose requires a prior model of the object while the proposed method does not. We also want to point out a recent similar work MidasTouch [Suresh+, 2022] also requires ground-truth mesh models of the target objects and requires a huge number of interactions for pose estimation than ours (1800 vs 10).

[Assembly after localization]
Once TactileFilter localizes the hole and finds the correct peg, we treat the peg insertion task as a pick-and-place task. The mating parts have a tolerance of 2 mm and a simple pick and place with an impedance controller succeeds in insertion. Our primary objective in this study is to identify and estimate the pose of mating parts, not to resolve any contact formation during assembly. To do tighter assembly, we can use some prior work along with our method, such as [13,20].

[Sim2Real]
We understand and acknowledge the shortcoming of real data collection of our method, and we had already mentioned it as future work in our manuscript. The current simulators [9,34,35] do not support GelSight Mini and we are working towards developing one.

[Computation cost]
Computing importance weights for action generation (Eq.2) and localization (Eq.4) takes approximately 0.3 seconds on a single GPU.

[Test on small objects]
We cannot resolve the pose uncertainty from single touch in case of partial overlap between the sensor and small objects. As presented in Table 1, a single touch yields only 59.1\% accuracy, primarily because many objects share a similar contact patch, necessitating multiple touches to resolve the ambiguity.

[MAZE board for training]
We use the MAZE board to collect data for training our part-mating model using contrastive learning. This allows us to design a generalizable model that can identify completely novel parts that fit together (all the alphabet characters and industrial connectors we use in experiments were never used for training).

["previously collected images"]
As stated in our manuscript, we collect data for the pegs before conducting online experiments, which corresponds to the "Offline data collection" depicted in Fig. 1. We use these images to compute likelihoods (weights) during the hypothesis updating stage.

[Raspberry Pi experiment]
We apologize for the confusion. In the revised paper, we will include the results of TactileFilter in this experiment to provide a complete evaluation of the proposed approach.

[Baseline]
We define the baseline to be single touch because the closest work to ours, Tac2Pose, only considers single touch. We want to emphasize that Tac2Pose assumes prior knowledge of 3D geometry of the parts while we do not. The Pixel baseline performs better in the large dataset because the number of objects is smaller in the large dataset than in the small dataset (24 vs 12).

[Submilimeter accuracy]
The error in SE(2) shown in Table I and II have averaged errors over different initial poses (4200 for small and 10164 for large objects). The current method is not expected to work in the continuous domain since we assume no prior knowledge of geometry.


\clearpage
\subsection{Author feedback -- factual errors or substantive misunderstandings --}
We apologize for any confusion caused by defining the task as "multi-object assembly". Assembly would be a suitable application of our method, but we would like to emphasize that this research primarily focuses on the simultaneous identification and localization of parts that fit together.
The novelty of our proposed method is to bring together contrastive learning, particle filtering, and tactile perception while minimizing the number of interactions during perception. We believe such a work has not appeared in open literature before. Any contact interaction during assembly is not considered in this task. However, this can be solved by combining some prior work (ref [10,12]) with our proposed method.

[Novelty]
We respectfully assert the proposed algorithm is novel and addresses a distinctive and important robotic problem. In summary, our contributions can be outlined as follows:

1. We investigate a general-purpose part mating problem, where the shapes of the objects are not known a priori, and the task is to identify and estimate the pose of the mating parts with a minimum number of interactions.

2. Our combination of the learning-based part mating model and particle filter is novel and is supported by empirical evidence that demonstrates its ability to disambiguate its beliefs through interactions. Additionally, the proposed action selection method yields significant improvements in efficiency. Furthermore, our algorithm is evaluated on novel objects, which can show generalization to unseen objects, while the closest work Tac2Pose assumes it has access to the ground-truth 3D geometry.

[Contrast to prior work]
TacTip [Lepora+, 2019], pointed out by the meta reviewer, considers a problem of edge perception and contour following. Since our primary objective is to identify and localize novel parts that fit together, we cannot compare to this method.
In terms of generalization to unknown objects, prior pose estimation method using tactile sensors, Tac2Pose [Bausa+, 2021], MidasTouch [Suresh+, 2022], auto-encoder-based [Caddeo+, 2023], and RL-based [Kelestemur+, 2022] models assume prior knowledge of ground-truth 3D meshes and/or use of a simulator, which limit their applications to novel objects. Our method generalizes to unknown geometries as shown in the experiments (small/large objects and industrial connectors are not used for training the contrastive learning model).
In terms of using particle filtering, [Luo+, 2015] localizes interaction locations using multiple contacts obtained by a low-resolution (14x6) tactile sensor and thus cannot capture fine details of objects that are essential for fine-grained identification and localization tasks demonstrated in our paper (we use the GelSight Mini whose resolution is 320x240x3). MidasTouch [Suresh+, 2022] also uses multiple touches to update hypotheses, however, it uses a much higher number of interactions compared to our method (1800 vs 10), and assumption to have access to ground-truth 3D geometry. Furthermore, both works assume the next action is given, while TactileFilter selects an optimal action by finding the most informative action using a trained contrastive learning model, and we empirically showed it significantly improves performance compared to random action.

[Number of objects in small/large test settings]
We apologize for the misunderstanding by reducing the number of alphabets from 24 to 12 in the "large" setting. In reality, robots do not often encounter situations where they need to identify parts from 24 different categories, as demonstrated in the connectors and sockets mating task in Figure 7 (6 sockets in total on the Raspberry Pi board). As a result, we will reduce the number of alphabets in the "small" setting to 12 to maintain consistency between the two settings. The classification accuracy on the different numbers of objects (4, 8, 12) can be seen in Figure 5, which shows the algorithm takes more interactions to reduce ambiguity if the number of objects increases.
